Tempo: Accelerating Transformer-Based Model Training through Memory Footprint Reduction

Training deep learning models can be computationally expensive. Prior works have shown that increasing the batch size can potentially lead to better overall throughput. However, the batch size is frequently limited by the accelerator memory capacity due to the activations/feature maps stored for the training backward pass, as larger batch sizes require larger feature maps to be stored. Transformer-based models, which have recently seen a surge in popularity due to their good performance and applicability to a variety of tasks, have a similar problem. To remedy this issue, we propose Tempo, a new approach to efficiently use accelerator (e.g., GPU) memory resources for training Transformer-based models. Our approach provides drop-in replacements for the GELU, LayerNorm, and Attention layers, reducing the memory usage and ultimately leading to more efficient training. We implement Tempo and evaluate the throughput, memory usage, and accuracy/loss on the BERT Large pre-training task. We demonstrate that Tempo enables up to 2x higher batch sizes and 16% higher training throughput over the state-of-the-art baseline. We also evaluate Tempo on GPT2 and RoBERTa models, showing 19% and 26% speedup over the baseline.

==> sections/4-ImplementationDetails.tex <==
\section{Implementation Details}
\label{sec:Implementation_Details}

\subsection{In-Place GELU}
    As we show in Section~\ref{sec:Key_Ideas}, it is possible to compute the inverse of the GELU function by knowing what side of the minimum the input originated from. This is shown in Equation \ref{eq:gelu_inverse} where $\operatorname{GELU*}$ is a function that returns both the $\operatorname{GELU}$ output and $m$ is the mask bit that denotes which side of the minimum the input originates from.
    \begin{equation} \label{eq:gelu_inverse}
        \operatorname{GELU*}^{-1} (\operatorname{GELU}(x), m) = x
    \end{equation}
    
   Moreover, we observe that we do not need to compute the inverse and then compute the derivative with respect to the input in a two step process as a na\"{i}ve approach would suggest. Instead, we can precompute this composition (see Equation \eqref{eq:gelu_compose}):
    \begin{equation} \label{eq:gelu_compose}
        \frac{d \operatorname{GELU}}{dx}(y) = \operatorname{GELU}' \circ \operatorname{GELU*}^{-1} (y, m)
    \end{equation}
    in order to \textbf{compute the derivative with respect to the input} directly using the output value. A plot of this relationship is shown in Figure~\ref{fig:gelu_derivative}. 
    
    
    \begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.495\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{Images/gelu_derivative_large.png}
        \caption{GELU derivative from \eqref{eq:gelu_compose}. The section corresponding to $x > -0.75179$ is in blue, $x \leq -0.75179$ -- in orange.}
        \label{fig:gelu_derivative}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\columnwidth}
        \centering
         \includegraphics[width=\columnwidth]{Images/gelu_deriv_approx_large.png}
        \caption{Our approximation of function \eqref{eq:gelu_compose} with a piece-wise polynomial approximation. Different sections of the approximation are shown in different colours.}
        \label{fig:ourgeluderiv}
    \end{subfigure}
    \end{figure}
    
    A key observation about the GELU function is that it is transcendental, and hence there is no simple solution for the inverse of the GELU function in terms of elementary functions~\cite{transcendental}. We therefore approximate sections of Equation~\eqref{eq:gelu_compose} with a piece-wise polynomial with a degree up to 13.\footnote[4]{Additional details of this implementation are covered in Appendix \ref{appdix:ImplDetails}.} A plot of this approximation is shown in Figure~\ref{fig:ourgeluderiv}. 
    
\subsection{In-Place LayerNorm}
    As stated in Section \ref{sec:Key_Ideas}, we aim to reuse the output of the LayerNorm \cite{layernorm}, which must be stored for the backpropagation of the successive fully-connected layers, while discarding the input. Although prior work has demonstrated the usability of In-Place Activated BatchNorm in the context of CNN networks \cite{rotabulo2017}, we note that this approach is not applicable in the Transformer case, which employs LayerNorm instead~\cite{vaswani2017}.
    
    By employing an alternative derivation for the gradient of LayerNorm which stashes alternative parameters, we can compute the gradients with \emph{negligible} performance overhead while achieving ideal memory footprint reduction for this operator. Following a similar approach as for In-Place GELU, we implement this operator as a Python PyTorch module, allowing it to be easily substituted in place of the existing LayerNorm layer in an implementation of the BERT model~\cite{deeplearningexamples, huggingface}. See \ref{appdix:ImplDetails} for additional implementation details and the full derivation.
    
\subsection{Sub-Layer Dropout Recomputation}

    Our basic implementation of Sub-Layer Dropout Recomputation follows the example of our other optimizations. Note that the way Dropout is implemented requires a randomly generated mask, where a portion of the inputs are set to zero according to a percentage $p$, which is also needed in the backward pass~\cite{pytorch, mxnet}. We simply stash this mask and discard the output. Then, in the backward pass, we recompute the output as shown in Figure \ref{fig:dropout}. Storing a boolean mask of size $N$ will take $N \times 1$ bytes, boolean tensors in PyTorch use 1 byte per value, while 32-bit floating points will use $N \times 4$ bytes~\cite{pytorch}. Therefore, the total memory saved by discarding the output will be $4/5$ of the total pre-optimization dropout output memory cost.
    
    In contrast to prior works which modify the framework and may not expose this optimization \cite{capuchin, dtr_implementation, checkmate_implementation}, we develop a PyTorch module which can be added to reduce the memory pressure of the critical attention section of the Transformer-based models~\cite{vaswani2017} with minimal overhead. Appendix \ref{appdix:ImplDetails} provides more in-depth comparison between prior work and our implementation.
    

\subsection{Other Engineering Optimizations}
We note that PyTorch uses a memory-inefficient implementation of the softmax function which retains both the input and output of the function for the backward pass \cite{pytorch}. Instead, only the output is necessary. This optimization has also previously been implemented as part of some models in the Huggingface library \cite{deberta_huggingface}. We use this optimization as well in our implementation of the attention mechanism to further reduce the activation memory pressure.

==> sections/6-Related_Works.tex <==
\section{Related Works}
\label{sec:Related_Works}

There has been a number of previous works~\cite{Sanh2019DistilBERTAD, jiao-etal-2020-tinybert, longformer, performer, big-bird} which focus on developing models that remain competitive with BERT and other Transformer-based models while requiring less memory and compute. One approach that has been taken is to tackle the $\mathcal{O}(S^2)$ nature of the attention mechanism \cite{survey}. Out of these, a few interesting and relevant ideas in terms of memory footprint reduction involve sparsifying the attention mechanism \cite{longformer, big-bird}, or using a decomposable softmax layer in order to avoid doing the $\mathcal{O}(S^2)$ computation in the first place \cite{performer}. In contrast, our technique targets a broad spectrum of sequence lengths. Other models such as TinyBERT \cite{jiao-etal-2020-tinybert} and DistilBERT \cite{Sanh2019DistilBERTAD} take a different approach in reducing the total model size. In these works, the technique of \textit{Distillation} is used to train a smaller student network from a larger teacher network \cite{HinVin15Distilling}. These approaches are model-level algorithm changes, and therefore orthogonal to our work.

% \subsection{General Memory Footprint Reduction Techniques}

% We expand on the techniques we referred to in section \ref{sec:Background_and_Motivation} in this section. As previously iterated in section \ref{sec:Background_and_Motivation}, (1) these techniques do not look closely at the specific structure of the BERT model, (2) At a per layer level, our techniques can provide better performance at a cheaper computational cost, and (3) these techniques are orthogonal to our work.

% \subsubsection{Checkpointing}

% Early work in this direction was able to reduce the memory cost of linear models to $\mathcal{O}(\sqrt{n})$ for general linear models in the number of layers. Further work  has expanded on this. Echo has innovative optimizations for specific models \cite{zheng2020}, Checkmate computes an optimal checkpointing schedule minimizing recomputation time with respect to a specific memory budget \cite{checkmate}, and Dynamic Tensor Rematerialization uses online heuristics to minimize recomputation time while training \cite{dtr}. Furthermore, there are works in this area that combine checkpointing with other technniques such as offloading detailed below.

% \subsubsection{Offload}

% Initial work in this direction such as vDNN focused on specific schemes to offload layer outputs depending on their computation cost \cite{vdnn}. There was also some consideration into prefetching feature maps in anticipation of their use in the backward pass. More work in that direction focuses on several different directions. For one, Superneurons \cite{superneurons} combines both checkpointing and offloading. In this work, they checkpoint computationally cheap layers, avoiding transfer overhead, while simultaneously offloading computationally expensive layers, avoiding recomputation overhead for those cases. Capuchin takes this further in considering tensor level accesses, as well as considering the runtime fetching and computation time in making decisions on which strategy to apply \cite{capuchin}. Additonally, ZeRO-Infinity combines offloading of feature maps with offloading of model states and other optimizations \cite{zeroinf}.

% \subsubsection{Compression}

% Works like Gist \cite{jain2018} and ActNN \cite{actnn} both include forms of lossy compression. Gist specifically targets CNN based models with a variety of different lossy and lossless optimizations, taking an approach similar to our own in examining the model structure closely \cite{jain2018}. However, as this is a work focused on CNNs, the techniques described do not directly apply to the BERT model we are aiming to optimize for. ActNN on the other hand is a more general technique, using a quantization strategy designed to reduce the number of bits needed for feature map storage, while preserving certain theoretical guarantees regarding model conversion \cite{actnn}. It additionally shows good performance relative to techniques such as Dynamic Tensor Rematerialization \cite{dtr} and Capuchin \cite{capuchin}. This work does not consider the BERT model however \cite{actnn}.


Two other important techniques are mixed-precision training~\cite{mixed} and in-place activated BatchNorm~\cite{rotabulo2017}. Mixed precision training involves training using both 32-bit and 16-bit IEEE floating point numbers depending on the numerical sensitivity of different layers \cite{mixed}. This both decreases the training time and the memory pressure of the model dependent on the hardware \cite{mixed}. Reversible BatchNorm uses techniques designed to optimize the memory footprint of CNN models which make extensive use of RELU and BatchNorm operators \cite{rotabulo2017}. They do this by deriving in-place expressions for these operators (the input feature map for these operators no longer needs to be stored). Although this work shows better performance than checkpointing, it is also specific to CNN models, so is not directly comparable to our work. Other recent works such as Substation~\cite{datamovement} aims to improve training performance by reducing the total movement of data with operator fusion; this is also orthogonal to our memory footprint-based approach.

Other techniques are more focused on inference and model weights, both of which are not applicable in this context of Transformer-based model \emph{training}, where the \emph{activations} are the memory bottleneck \cite{deepcompression, eie, eyeriss, conciseload, cnvlutin, diannao, stripes, scnn, scaledeep}.

==> sections/9-Availability.tex <==
%-------------------------------------------------------------------------------
\section{Availability}
\label{Availability}
%-------------------------------------------------------------------------------

We open-source \emph{Tempo} for an immediate positive impact on both machine learning researchers and practitioners here: \url{https://github.com/UofT-EcoSystem/Tempo}.
%-------------------------------------------------------------------------------
